Learning to Design Circuits

Analog IC design relies on human experts to search for parameters that satisfy circuit specifications with their experience and intuitions, which is highly labor intensive, time consuming and suboptimal. Machine learning is a promising tool to automate this process. However, supervised learning is difficult for this task due to the low availability of training data: 1) Circuit simulation is slow, thus generating large-scale dataset is time-consuming; 2) Most circuit designs are propitiatory IPs within individual IC companies, making it expensive to collect large-scale datasets. We propose Learning to Design Circuits (L2DC) to leverage reinforcement learning that learns to efficiently generate new circuits data and to optimize circuits. We fix the schematic, and optimize the parameters of the transistors automatically by training an RL agent with no prior knowledge about optimizing circuits. After iteratively getting observations, generating a new set of transistor parameters, getting a reward, and adjusting the model, L2DC is able to optimize circuits. We evaluate L2DC on two transimpedance amplifiers. Trained for a day, our RL agent can achieve comparable or better performance than human experts trained for a quarter. It first learns to meet hard-constraints (eg. gain, bandwidth), and then learns to optimize good-to-have targets (eg. area, power). Compared with grid search-aided human design, L2DC can achieve $\mathbf{250}\boldsymbol{\times}$ higher sample efficiency with comparable performance. Under the same runtime constraint, the performance of L2DC is also better than Bayesian Optimization.

==> texts/figures/figure1.tex <==
\begin{figure}[ht]
        \centering
        \subfigure[\label{fig:env1sch}]{\includegraphics[width=0.48\columnwidth, height=0.36\columnwidth]{images/schematic/env1sch.pdf}}
        \subfigure[\label{fig:env1curve}]{\includegraphics[width=0.48\columnwidth,height=0.36\columnwidth]{images/programmed/one/curve.pdf}}
        \caption{\ref{fig:env1sch} Schematic of one-stage voltage amplifier. We set $W3 = W4, L3 = L4$ and $W5 = W6, L5 = L6$ for the circuit symmetry. \ref{fig:env1curve} Learning curves of one-stage amplifier. Although random can get better score than human, it cannot outperform DDPG.}
\end{figure}

==> texts/figures/figure2.tex <==
\begin{figure*}[!ht]
        \centering
        \subfigure[\label{fig:env2sch}]{\includegraphics[width=0.48\columnwidth, height=0.36\columnwidth]{images/schematic/env2sch.pdf}}
        \subfigure[\label{fig:env2curve}]{\includegraphics[width=0.48\columnwidth, height=0.36\columnwidth]{images/programmed/two/curve.pdf}}
        \caption{\ref{fig:env2sch} Schematic of Two-stage voltage amplifier. We set W3 = W4, L3 = L4, W5 = W6, L5= L6 for the circuit symmetry. \ref{fig:env2curve} Learning curves of two-stage voltage amplifier. DDPG can outperform human design with only about 8k simulations. Random search is far from beating human design.}
        \vspace{-12pt}
\end{figure*}

==> texts/tables/setup.tex <==
\begin{table}[]
    \centering
    \caption{\label{tab:setup}Setups for four environments}
    \begin{tabu}{l|cccc}
        \tabucline[1pt]{-}
        & \begin{tabular}[c]{@{}c@{}}One-stage\\ Voltage Amplifier\end{tabular} & \begin{tabular}[c]{@{}c@{}}Two-stage\\ Voltage Amplifier\end{tabular} & \begin{tabular}[c]{@{}c@{}}Three-stage\\ transimpedance\\Amplifier\end{tabular} & \begin{tabular}[c]{@{}c@{}}Two-stage \\transimpedance\\Amplifier \end{tabular}\\\hline
        $W$ search space & $[0.35~\mathrm{\mu m}$, $500~\mathrm{\mu m}]$ & $[120~\mathrm{nm}$, $1000~\mathrm{nm}]$ & $[2~\mathrm{\mu m}, 10~\mathrm{\mu m}]$ & $[0.18~\mathrm{\mu m}, 10~\mathrm{\mu m}]$ \\
        $L$ search space & $[0.35~\mathrm{\mu m}$, $2~\mathrm{\mu m}]$ & $[60~\mathrm{nm}$, $1000~\mathrm{nm}]$ &  $[1~\mathrm{\mu m}$, $2~\mathrm{\mu m}]$ & $=1~\mathrm{\mu m}$ \\
        Optimization targets & power, gate area & power, gate area & power, gate area & bandwidth \\
        $\alpha$ & 0 & 1 & 0 & 1\\
        $e_0$ & -2 & -5 & -2 & -6 \\
        $e_1$ & 0 & -2 & 0 & 0 \\
        $ T $ & 5 & 3 & 5 & 5\\
        \begin{tabular}[l]{@{}l@{}}DC operation observations\end{tabular} & 8 & 32 & 12 & 6 \\
        \begin{tabular}[l]{@{}l@{}}Magnitude response dim\end{tabular} & 10001 & 436 & 8001 & 4001 \\
        \begin{tabular}[l]{@{}l@{}}Phase response dim\end{tabular} & 10001 & 436 & 8001 &4001 \\
        \begin{tabular}[l]{@{}l@{}}Magn-phase embed dim\end{tabular} & 30 & 50 & 50 & 50 \\
        Local transistor observations & 22 & 96 & 22 & 22 \\
        Simulation tool & hspice & spectre & hspice & hspice\\ 
        \tabucline[1pt]{-}
    \end{tabu}
\end{table}

==> texts/tables/table1.tex <==
\begin{table*}[ht]
    \small
    \centering
    \caption{\label{tab:env1result} In the simple environment one-stage amplifier, DDPG consumes lowest power and gate area to meet gain and unity gain bandwidth hard-constraints.}
    \begin{tabu}{c|c|cc|cc|c}
        \tabucline[1pt]{-}
             & \begin{tabular}[c]{@{}c@{}}Number of \\ Simulations\end{tabular} & \begin{tabular}[c]{@{}c@{}}Unity Gain \\ Bandwidth ($\mathrm{MHz}$)\end{tabular}  & Gain & Power ($\mathrm{mW}$) & Gate Area ($\mathrm{{\mu m}^2}$) & Score \\
        \hline
            Spec(Human)  & -- & 191 & 51.1 & 6.58 & 524 & 2.00 \\
        \hline
            Random  & 16,000 &  216 & \textbf{85.5} & 4.47 & 190 & 4.22 \\
        \hline
            DDPG   & 16,000 & \textbf{229}  & 56.2 & \textbf{4.11} & \textbf{165} & \textbf{4.78} \\
        \tabucline[1pt]{-}
    \end{tabu}
\end{table*}

==> texts/tables/table2.tex <==
\begin{table*}[!ht]
    \small
    \centering
    \caption{\label{tab:env2result}In a more complicated two stage voltage amplifier environment, random can on longer meet hard-constraints as marked in red. DDPG outperforms human expert in all the five performance metrics.}
    \begin{tabu}{c|c|ccc|cc|c}
    \tabucline[1pt]{-}
       & \begin{tabular}[c]{@{}c@{}}Number of \\ Simulations\end{tabular} & \begin{tabular}[c]{@{}c@{}}Unity Gain \\ Bandwidth\\ ($\mathrm{MHz}$) \end{tabular} & \begin{tabular}[c]{@{}c@{}}Phase \\ Margin ($\mathrm{^\circ}$)\end{tabular} & Gain ($\times 10^2$) & \begin{tabular}[c]{@{}c@{}} Power\\ ($\mathrm{nW}$)\end{tabular} & \begin{tabular}[c]{@{}c@{}} Gate Area \\ ($\times 10^5~\mathrm{nm^2}$)\end{tabular} & Score \\
    \hline
        \begin{tabular}[c]{@{}c@{}} Spec\\(Human) \end{tabular}  & -- & 102 & 58 & 5.71 & 3390 & 19.3 & 2.00  \\
    \hline
        Random  & 30,000 & {\color{red}74.8} & 61 & 9.32 & 223 & 18.3 & -0.14 \\
    \hline
        DDPG  & 30,000 & \textbf{104} & \textbf{64} & \textbf{8.16} & \textbf{969} & \textbf{9.22} & \textbf{3.59} \\
    \tabucline[1pt]{-}
    \end{tabu}
\end{table*}
